Cognitive TransFuser: Semantics-guided Transformer-based Sensor Fusion for Improved Waypoint Prediction

Sensor fusion approaches for intelligent self-driving agents remain key to driving scene understanding given visual global contexts acquired from input sensors. Specifically, for the local waypoint prediction task, single-modality networks are still limited by strong dependency on the sensitivity of the input sensor, and thus recent works therefore promote the use of multiple sensors in fusion in feature level in practice. While it is well known that multiple data modalities encourage mutual contextual exchange, it requires global 3D scene understanding in real-time with minimal computation upon deployment to practical driving scenarios, thereby placing greater significance on the training strategy given a limited number of practically usable sensors. In this light, we exploit carefully selected auxiliary tasks that are highly correlated with the target task of interest (e.g., traffic light recognition and semantic segmentation) by fusing auxiliary task features and also using auxiliary heads for waypoint prediction based on imitation learning. Our RGB-LIDAR-based multi-task feature fusion network, coined Cognitive TransFuser, augments and exceeds the baseline network by a significant margin for safer and more complete road navigation in the CARLA simulator. We validate the proposed network on the Town05 Short and Town05 Long Benchmark through extensive experiments, achieving up to 44.2 FPS real-time inference time.

==> feedback.tex <==
% rita feedback

% 1. abstract can be improved by mentioning the overall overview of the paper. Current abstract is not covering the whole paper discussion -> O
% 2. why not mention cognitive transfuser in the title and abstract -> O
% 3. the reference should be cited in consecutive order from 1,2,3... -> O
% 4. fig. 3: detailed reason of using STDC-Seg -> O
% 5. The experimental results 4.3: add visualisation of data. -> X
% 6. lengthy -> succinct

% - More details on the TransFuser number and configuration of transformer blocks used for RGB and LiDAR fusion. -> O
% - The pre-training process and datasets used for the semantic segmentation and traffic
% light recognition models could be described in a bit more detail. -> partial O
% - The evaluation results could be discussed a bit more, especially analyzing why early
% fusion of semantic features outperformed other fusion approaches.
% - The work could be situated more clearly in relation to other recent methods for sensor
% fusion and autonomous driving. How does it compare to other multi-modal, multi-task
% approaches? -> X (already in table?)
% - Additional results could be provided, such as sample qualitative predictions to
% demonstrate where the proposed method improves over the baseline. -> X (can't)
% - Limitations and future work could be discussed, such as how the approach could be
% extended to incorporate other sensory modalities or tasks. -> O
% - More analysis could be provided on the tradeoffs between performance gains and
% computational overhead when adding the auxiliary tasks.


% 1. Fig.1 was not mentioned until section §4.2 (page 7). Font sizes of some texts could be
% increased. The author could also consider to label the Heads next to their dimension to
% help the reader. -> O
% 2. A visualized example of the 2-bin histogram mentioned in §3.2 would be helpful.
% 3. §4.1, last sentence of first paragraph was confusing for me as it mentioned Figs.2&3
% together, so I expected to see corresponding features in Fig.3 processed from Fig.2.
% Whereas Fig.3 seems to be just an example of semantic segmentation result. -> O
% 4. Denotations of TL and SS were only mentioned in Table 1. It might help to mention them
% in main text as well. -> X (already mentioned elsewhere)
% 5. In §4.3, it would help if the author could put numbers behind the descriptions of the
% results., to guide the readers through Table1. ->


